Combinatorial Persistent Homology Transform

The combinatorial interpretation of the persistence diagram as a M\"obius inversion was recently shown to be functorial. We employ this discovery to recast the Persistent Homology Transform of a geometric complex as a representation of a cellulation on $\mathbb{S}^n$ to the category of combinatorial persistence diagrams. Detailed examples are provided. We hope this recasting of the PH transform will allow for the adoption of existing methods from algebraic and topological combinatorics to the study of shapes.

==> body/cosheaf-pipeline.tex <==
Let $X$ be a topological space that admits a cellulation.

\paragraph{Filtration Cosheaf}
Fix a topological space $X$ that admits a cellulation.


\begin{defn}
Let $\Fil(X)$ be the category whose objects are tuples $(\Sstrat, \Ffunc)$ where
$(X, \Sstrat)$ is a cellulation and $\Ffunc : \Ent(X, \Sstrat) \to \Fil$ is a cellular
cosheaf of filtrations.
A morphism $\alpha : (\Sstrat, \Ffunc) \to (\Tstrat, \Gfunc)$ is a cellular map
$\alpha : (X, \Sstrat) \to (X, \Tstrat)$ such that for all $\sigma \in \Tstrat$,
$\Gfunc(\sigma) = \colim \, \Ffunc |_{\alpha^{-1}(\sigma)}.$
\end{defn}

\todo{check composition to make sure this is actually a category}

\paragraph{Monotone Integral Functions Cosheaf}
\todo{graded cellular cosheaves over $X$ valued in $\Mon$.}

Fix a topological space $X$ that admits a cellulation.

\begin{defn}
Let $\Mon(X)$ be the category whose objects are tuples $(\Sstrat, \Ffunc)$ where
$(X, \Sstrat)$ is a cellulation and $\Ffunc : \Ent(X, \Sstrat) \to \Mon$ is a cellular
cosheaf of filtrations.
A morphism $\alpha : (\Sstrat, \Ffunc) \to (\Tstrat, \Gfunc)$ is a cellular map
$\alpha : (X, \Sstrat) \to (X, \Tstrat)$ such that for all $\sigma \in \Tstrat$,
$\Gfunc(\sigma) = \colim \, \Ffunc |_{\alpha^{-1}(\sigma)}.$
\end{defn}

\todo{check composition to make sure this is actually a category}


\paragraph{Integral Functions Cosheaf}
\todo{graded cellular cosheaves over $X$ valued in $\Fnc$.}
Fix a topological space $X$ that admits a cellulation.

\begin{defn}
Let $\Fnc(X)$ be the category whose objects are tuples $(\Sstrat, \Ffunc)$ where
$(X, \Sstrat)$ is a cellulation and $\Ffunc : \Ent(X, \Sstrat) \to \Fnc$ is a cellular
cosheaf of filtrations.
A morphism $\alpha : (\Sstrat, \Ffunc) \to (\Tstrat, \Gfunc)$ is a cellular map
$\alpha : (X, \Sstrat) \to (X, \Tstrat)$ such that for all $\sigma \in \Tstrat$,
$\Gfunc(\sigma) = \colim \, \Ffunc |_{\alpha^{-1}(\sigma)}.$
\end{defn}

\todo{check composition to make sure this is actually a category}


==> body/main-theorem.tex <==
\todo{...}


==> body/pht_functor.tex <==
Fix a finite simplicial complex $K$ and let $K^0 \subseteq K$ its subset of vertices.
Let $\Sspace^N := \{ \mu \in \Rspace^{N+1} : ||\mu|| = 1 \}$ the sphere of all directions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{PL Embeddings}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Recall, a PL embedding of $K$ into $\Rspace^{N+1}$ 
is completely determined by its values on $K^0$.
That is, given a PL embedding $\phi : |K| \to \Rspace^{N+1}$, a simplex 
$\sigma = [v_0, \cdots, v_k]$, and a point $x \in | \sigma |$,
$$\phi(x) = t_0 \phi(v_0) + \cdots + t_k \phi (v_k),$$
where $(t_0, \cdots, t_k)$ are the barycentric coordinates of $x$.
For every subset $S \subseteq K^0$, denote by $\aff_\phi(S) \subseteq \Rspace^{N+1}$ 
the affine hull of the set of points $\big \{ \phi (v) \big \}_{v \in S}$.

Fix a PL embedding $\phi : |K| \to \Rspace^{N+1}$.
Let $E := \{ e = (v, v') : v, v' \in K^0 \}$ be the set of all unordered, distinct pairs
of vertices.
For every $e = (v, v')$ in~$E$, there is a unique line $\ell_e \subseteq \Rspace^{N+1}$
connecting the two points $\phi(v)$ and $\phi(v')$.
For every such line~$\ell_e$, there is a unique $N$-dimensional linear subspace
$H_e \subseteq \Rspace^{N+1}$ perpendicular to $\ell_e$ and intersecting the
origin. \brittany{to me, skipping $\ell_e$ is more natural and uses less
notation}
The intersection $S_e := H_e \cap \Sspace^{N}$ is a great $(N-1)$-sphere.
By the Jordan-Brouwer separation theorem, $\Sspace^{N} \setminus S_e$
has two connected components (sides) denoted arbitrarily by $S_e^+$ and~$S_e^-$;
see~\cite{lebesgue1911,brouwer1911} \todo{cite modern textbook}.
Let~$\Acal_\phi := \{ S_e : e \in E\}$ be the multiset of all such great
$N$-spheres.
We call $\Acal_\phi$ a signed \emph{arrangement} of spheres.
The signed arrangement $\Acal_\phi$ is \emph{essential}
if the following condition holds: $\bigcap_{e \in \Acal_\phi} S_e = \emptyset$.


Now consider two PL embeddings $\phi, \psi : |K| \to \Rspace^{N+1}$ such that both
arrangements $\Acat_\phi$ and $\Acat_\psi$ are essential.
We say $\psi$ is a \emph{specialization} of $\phi$, written $\psi \preceq \phi$, if for every subset
$S \subseteq K^0$, $\dim \aff_\phi(S) \leq \dim \aff_\psi(S)$.
If $\upsilon \preceq \psi$ and $\psi \preceq \phi$, then $\upsilon \preceq \phi$.

\begin{defn}
Let $\PL(K, \Rspace^{N+1})$ be the category whose objects
are PL embeddings $\phi : |K| \to \Rspace^{N+1}$ such that $\Acat_\phi$ is essential 
and whose morphisms are specializations $\preceq$.
\end{defn}

Note that if $\psi \preceq \phi$ and $\phi \preceq \psi$, then $\phi \cong \psi$.
For example, if $\phi$ is a translation or rotation of $\psi$, then $\phi \cong \psi$.
Further, the skeleton of $\PL(K, \Rspace^{N+1})$ is a poset.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Cellular Cosheaves of Filtrations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $\S^N$ be the topological $N$-sphere.
A \emph{cellular cosheaf of filtrations} over $(\S^N, \Sstrat)$, or simply an 
$\Sstrat$-cosheaf of filtrations, is a functor $F : \Sstrat \to \Fil(K)$.
Given a cellular specialization $\alpha : (\S^N, \Sstrat) \to (\S^N, \Tstrat)$ and a cosheaf
$F$ over $(X, \Sstrat)$, its push-forward $\alpha_\ast F : \Tstrat \to \Fil(K)$
is the cellular cosheaf that assigns to every cell $C \in \Tstrat$, the filtration
$\colim \, F \big( \alpha^{-1}(C) \big)$ and to every face relation $C_1 \leq C_2$
the canonical filtration-preserving morphism 
$$\alpha_\ast  F (C_1 \leq C_2) : \alpha_\ast F (C_2) \to \alpha_\ast F (C_1)$$
induced by the universal property of the colimit.
A \emph{morphism} from an $\Sstrat$-cosheaf $F$ to a $\Tstrat$-cosheaf $G$ is a 
cellular specialization $\alpha : \Sstrat \to \Tstrat$ such that $G = \alpha_\ast F$.

\begin{defn}
Let $\Csh \big( \S^N, \Fil(K) \big)$ be the category whose objects are cellular
cosheaves valued in $\Fil(K)$, over all cellulations $(\S^N, \Sstrat)$ of the sphere,
and whose morphisms are triples $(F, G, \alpha)$ as described above.
\end{defn}


We now give a brief introduction to cellular cosheaves introducing only
those concepts we need.
See \cite{curry, shepard} for an introduction to cellular (co)sheaves, and see~\cite{curry_patel}
for an introduction to cosheaves constructible with respect to stratifications.

A \emph{topological cell} is a space homeomorphic to $\Rspace^n$ for some $n$.
A \emph{cell complex} $(X, \Sstrat)$ consists of a topological space $X$ and a partition
$\Sstrat$ of $X$ into disjoint topological cells~$\cup_{C \in \Sstrat} C = X$
such that if $X \cup \{ p \}$ is the one-point compactification of~$X$,
then $\cup_{C \in \Sstrat} C \cup \{ p \}$ are the cells of a regular CW complex
structure on $X \cup \{p \}$.
A \emph{cellulation} of a topological space $X$ is a cell complex $(X, \Sstrat)$.
The advantage of this definition of a cellulation is that many non-compact spaces of interest,
such as $\Rspace^n$, admit a finite cellulation.

Given a cell complex $(X, \Sstrat)$, its set of cells $\Sstrat$ has a natural partial order.
For two cells~$C_1, C_2 \in \Sstrat$, $C_1 \leq C_2$ if $C_1$ is a face of $C_2$.
A \emph{cellular cosheaf} on a cell complex $(X, \Sstrat)$ valued in a category $\Ccat$ is a functor
$\cosheaf{F} : \Sstrat \to \Ccat$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Cellular Cosheaves of Integral Functions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

